Synthetic Data for Deep Learning

Synthetic data is an increasingly popular tool for training deep learning models, especially in computer vision but also in other areas. In this work, we attempt to provide a comprehensive survey of the various directions in the development and application of synthetic data. First, we discuss synthetic datasets for basic computer vision problems, both low-level (e.g., optical flow estimation) and high-level (e.g., semantic segmentation), synthetic environments and datasets for outdoor and urban scenes (autonomous driving), indoor scenes (indoor navigation), aerial navigation, simulation environments for robotics, applications of synthetic data outside computer vision (in neural programming, bioinformatics, NLP, and more); we also survey the work on improving synthetic data development and alternative ways to produce it such as GANs. Second, we discuss in detail the synthetic-to-real domain adaptation problem that inevitably arises in applications of synthetic data, including synthetic-to-real refinement with GAN-based models and domain adaptation at the feature/model level without explicit data transformations. Third, we turn to privacy-related applications of synthetic data and review the work on generating synthetic datasets with differential privacy guarantees. We conclude by highlighting the most promising directions for further work in synthetic data studies.

==> applications.tex <==
\section{Applications of synthetic data in deep learning}\label{sec:direct}

In this section, we present an overview of recent works that use synthetic data directly, as a way to augment the dataset. We divide this part of the survey into subparts according to specific domains of application.

\subsection{General synthetic data approaches in computer vision}\label{sec:vision}

\subsubsection{Applications to general computer vision problems}\label{sec:visiongeneral}

...

A long line of work has used synthetic data for object detection. Peng et al.~\cite{Peng:2015:LDO:2919332.2920015} trained an object detection framework on non-realistic images of 3D models superimposed on real backgrounds, noting, in particular, that the results improve when synthetic data is varied along 3D pose, texture and color. Rajpura et al.~\cite{DBLP:journals/corr/RajpuraHB17} developed a Blender-based synthetic scene generator for recognizing objects inside a refrigerator, showing improved results with a fully convolutional version of GoogLeNet~\cite{7298594} adapted for object detection. \todo{MORE}

Segmentation \todo{MORE} Ward et al.~\cite{Ward2018DeepLS} improve leaf segmentation for \emph{Arabidopsis} plants for the CVPPP Leaf Segmentation Challenge by augmenting real data with a synthetic dataset produced with Blender. For a parallel challenge of leaf counting, Ubbens et al.~\cite{Ubbens2018} produce synthetic data based on an L-system plant model; they report improved counting results.

Another important class of applications for CGI-based synthetic data relates to problems such as 3D pose, viewpoint, and depth estimation, where manual labeling of real data is very difficult and sometimes close to impossible. Liebelt et al.~\cite{4587614} used 3D models to extract a set of 3D feature maps, then used a nearest neighbors approach to do multi-view object class detection and 3D pose estimation. \todo{MORE}

Easy variations and transformations provided by synthetic data can not only directly improve the results by training, but also represent a valuable tool for studying the properties of neural networks and other feature extractors. In particular, Pinto et al.~\cite{5711540} used synthetic data to study the invariance of different existing visual feature sets to variation in position, scale, pose, and illumination. Peng et al.~\cite{Peng2014ExploringII} and Pepik et al.~\cite{DBLP:journals/corr/PepikBRS15} used synthetic data to study the properties of deep convolutional networks, in particular robustness to various transformations, since synthetic data is easy to manipulate in a predefined way.

Earlier works recognized that the domain gap between synthetic and real images does not allow to expect state of the art results when training on synthetic data only, so many of them concentrated on bridging this gap by constructing hybrid datasets. V{\'a}zquez et al.~\cite{6587038} concentrated on pedestrian detection and proposed a scheme based on active learning: they initially train a detector on virtual data and then use selective sampling~\cite{Cohn1994} to choose a small subset of real images for manual labeling, achieving results on par with training on a large real datasets while using 10x less real data. 

Purely synthetic approaches were also used in early works, although mostly for problems where manual labeling would be even harder and noisier than for object detection or segmentation. The Render for CNN approach by Su et al.~\cite{7410665} outperformed real data with a hybrid synthetic+real dataset on the viewpoint estimation problem. Synthetic data helped improve 3D object pose estimation in Gupta et al.~\cite{DBLP:journals/corr/GuptaAGM15} and multi-view object class detection in Liebelt and Schmid~\cite{5539836} and Stark et al.~\cite{Stark2010BackTT}; as an intermediate step, the latter work used synthetic data to learn shape models. Hattori et al.~\cite{7299006} trained scene-specific pedestrian detectors on a purely synthetic dataset, superimposing rendered pedestrians onto a fixed real scene background.

An important question for direct applications is how realistic synthetic data must be in order to help with the underlying computer vision problem. Early works often argued that photorealism is not necessary for good domain transfer results; see, e.g.,~\cite{BMVC.28.82}. This question was studied in detail by Movshovitz-Attias et al.~\cite{10.1007/978-3-319-49409-8_18}. With the example of the viewpoint estimation problem for cars, they showed that photorealistic rendering does indeed help, showed that the gap between models trained on synthetic and real data can often be explained by domain adaptation (i.e., adapting from a different real dataset would be just as hard as adapting from a synthetic one), and hybrid synthetic+real datasets can significantly outperform training on real data only.

An interesting method of using synthetic data for object detection was proposed by Hinterstoisser et al.~\cite{10.1007/978-3-030-11009-3_42}. They note that training on purely synthetic data may give sub-par results due to the low-level differences between synthetic (rendered) images and real photographs. To avoid this, they propose to simply freeze the lower layers of, say, a pretrained object detection architecture and only train the top layers on synthetic data; in this way, basic features will remain suited for the domain of real photos while . Otherwise, this is a straightforward test of synthetic data: Hinterstoisser et al. superimpose synthetic renderings on randomly selected backgrounds and fine-tune pretrained Faster-RCNN~\cite{7485869}, R-FCN~\cite{DBLP:journals/corr/DaiLHS16}, and Mask R-CNN~\cite{8237584} object detection architectures with freezed feature extraction layers. They report that freezing the layers helps significantly, and different steps in the synthetic data generation pipeline (different domain randomization steps, see also Section~\ref{sec:domrand}) help as well, obtaining results close to training on a large real dataset.

...

Self-supervised multi-task learning~\cite{Ren2018CrossDomainSM}

...

3D position and orientation estimation for objects, known as the 6-DoF (degrees of freedom) pose estimation, is another important computer vision problem related to robotic grasping and manipulation. NVIDIA researchers Tremblay et al.~\cite{Tremblay2018DeepOP} approach it with synthetic data: using the synthetic data generation techniques we described in Section~\ref{sec:datahigh}, they train a deep neural network and report the first state of the art network for 6-DoF pose estimation trained purely on synthetic data. The novelty was that Tremblay et al. train on a mixture of domain randomized images, where distractor objects are placed randomly in front of a random background, and photorealistic images, where the foreground objects are placed in 3D background scenes obeying physical constraints; domain randomized images provide the diversity needed to cover real data (see Section~\ref{sec:domrand}) while realistic images provide proper context for the objects and are easier to transfer to real data.

...

Camera localization~\cite{8699232}

...


\subsubsection{Smart augmentation: compositing real data to produce synthetic datasets}\label{sec:cutpaste}

Another notable line of work that, in our opinion, lies at the boundary between synthetic data and data augmentation is to use combinations and fusions of different real images to produce a larger and more diverse set of images for training. This does not require the use of CGI for rendering the synthetic images, but does require a dataset of real images.

This field started in earnest with the \emph{Cut, Paste, and Learn} approach by Dwibedi et al.~\cite{Dwibedi2017CutPA}, which is based on the assumption that only \emph{patch-level realism} is needed to train, e.g., an object detector. They take a collection of object instance images, cut them out with a segmentation model (assuming that the instance images are simple enough that segmentation will work almost perfectly), and paste them onto randomized background scenes, with no regard to preserving scale or scene composition. Dwibedi et al. compare different classical computer vision blending approaches (e.g., Gaussian and Poisson blending~\cite{Perez:2003:PIE:882262.882269}) to alleviate the influence of boundary artifacts after the paste; they report improved instance detection results. The work on cut-and-paste was later extended with GAN-based models (used for more realistic pasting and inpainting) and continued in the direction of unsupervised segmentation by Remez et al.~\cite{Remez2018LearningTS} and Ostyakov et al.~\cite{DBLP:journals/corr/abs-1811-07630}.

Subsequent works extend this approach for generating more realistic synthetic datasets. Dvornik et al.~\cite{DBLP:journals/corr/abs-1807-07428} argue that an important problem for this type of data augmentation is to preserve visual context, i.e., make the environment around the objects more or less realistic. They describe a preliminary experiment where they placed segmented object at completely random positions in new scenes and not only did not see significant improvements for object detection on the VOC'12 dataset but actually saw the performance deteriorate, regardless of the distractors or strategies used for blending and boundary artifact removal. Therefore, they added a separate model (also a CNN) that predicts what kind of objects can be placed in a given bounding box of an image from the rest of the image with this bounding box masked out; then the trained model is used to evaluate potential bounding boxes for data augmentation, choose the ones with the best object category score, and then paste a segmented object of this category in the bounding box. The authors report improved object detection results on VOC'12. Wang et al.~\cite{Wang2019DataAF} develop this into an even simpler idea of \emph{instance switching}: let us switch only instances of the same class between different images in the training set; in this way, the context is automatically right, and shape and scale can also be taken into account. Wang et al. also propose to use instance switching to adjust the distribution of instances across classes in the training set and account for class importance by adding more switching for classes with lower scores. The resulting PSIS (Progressive and Selective Instance Switching) system provides improved results on the MS COCO dataset for various object detectors including Faster-RCNN~\cite{7485869}, FPN~\cite{8099589}, Mask R-CNN~\cite{8237584}, and SNIPER~\cite{NIPS2018_8143}.

\subsubsection{Domain randomization}\label{sec:domrand}

\emph{Domain randomization} is one of the most promising approaches to make straightforward transfer learning from synthetic data to real actually work. Consider a model that is supposed to train on $\dsyn\sim\psyn$ and later be applied to $\dreal\sim\preal$. The basic idea of domain randomization, first explicitly presented and named in~\cite{8202133}, is simple: let us try to make the synthetic data distribution $\psyn$ sufficiently wide and varied so that the model trained on $\psyn$ will be robust enough to work well on $\preal$.

Ideally, we would like to cover $\preal$ with $\psyn$, but in reality this is never achieved directly. Instead, synthetic data in computer vision can be randomized and made more diverse in a number of different ways at the level of either constructing a 3D scene or rendering 2D images from it:
\begin{itemize}
	\item at the scene construction level, a synthetic data generator (SDG) can randomize the number of objects, its relative and absolute positions, number and shape of distractor objects, contents of the scene background, textures of all objects participating in the scene, and so on;
	\item at the rendering level, SDG can randomize lighting conditions, in particular the position, orientation, and intensity of light sources, change the rendering quality by modifying image resolution, rendering type such as ray tracing or other options, add random noise to the resulting images, and so on.
\end{itemize}

The work~\cite{8202133} did the first steps to show that domain randomization works well; they used simple geometric shapes (polyhedra) as both target and distractor objects, random textures such as gradient fills or checkered patterns. The authors found that synthetic pretraining is indeed very helpful when only a small real training set is available, but helpful only if sufficiently randomized, in particular when using a large number of random textures. The approach was subsequently applied to a more ambitious domain by NVIDIA researchers Tremblay et al.~\cite{Tremblay2018TrainingDN}, who trained object detection models on synthetic data with the following procedure:
\begin{itemize}
	\item create randomized 3D scenes, adding objects of interest on top of random surfaces in the scenes;
	\item add the so-called ``flying distractors'', diverse geometric shapes that are supposed to serve as negative examples for object detection;
	\item add random textures to every object, randomize the camera parameters, lighting, and other parameters.
\end{itemize}
The resulting images were completely unrealistic, yet diverse enough that the networks had to concentrate on the shape of the objects in question. Tremblay et al. report improved car detection results for R-FCN~\cite{DBLP:journals/corr/DaiLHS16} and SSD~\cite{10.1007/978-3-319-46448-0_2} architectures (but failing to improve Faster R-CNN~\cite{7485869}) on their dataset compared to Virtual KITTI (see Section~\ref{sec:dataoutdoor}), as well as improved results on hybrid datasets (adding a domain-randomized training set to COCO~\cite{DBLP:journals/corr/LinMBHPRDZ14}), a detailed ablation study, and extensive experiments showing the effect of various hyperparameters.

By that point, domain randomization had operated under the assumption that realism is not necessary in synthetic data. Prakash et al.~\cite{Prakash2018StructuredDR} take the next logical step, continuing this effort to \emph{structured} domain randomization. They still randomize all of the settings mentioned above, but only within realistic ranges, taking into account the structure and context of a specific scene. MORE

\cite{Borrego2018ApplyingDR}

Tobin et al.~\cite{8593933} consider robotic grasping, a problem where the lack of data is especially dire (see also Sections~\ref{sec:rl} and~\ref{sec:darobot}). They use domain randomization to generate a wide variety of unrealistic procedurally generated object meshes and textured objects for grasping, so that a model trained on them would generalize to real objects as well. They show that a grasping model trained entirely on non-realistic procedurally generated objects can be successfully transferred to realistic objects.

\subsubsection{Improving CGI-based generation}\label{sec:cgi}

The basic workflow of synthetic data in computer vision is relatively straightforward: prepare the 3D models, place them in a controlled scene, set up the environment (camera type, lighting etc.), and render synthetic images to be used for training. However, some works on synthetic data present additional ways to enhance the data not by domain adaptation/refinement to real images (we will discuss this approach in Section~\ref{sec:domain}) but directly on the stage of CGI generation. In particular:
\begin{itemize}
	\item Wang et al.~\cite{DBLP:journals/corr/abs-1904-12294} recognize retail items in a smart vending machine; to simulate natural deformations in the objects, they use a surface-based mesh deformation algorithm proposed in~\cite{doi:10.3722/cadaps.2012.345-359}, introducing and minimizing a global energy function for the object's mesh that accounts for random deformations and rigidity properties of the material (Wang et al. also use GAN-based refinement, see Section~\ref{sec:synrefine});
	\item ...
\end{itemize}

...

\subsubsection{Synthetic data produced by generative models}\label{sec:datagan}

Generative models, especially Generative Adversarial Networks (GAN)~\cite{NIPS2014_5423}, are increasingly being used for domain adaptation, either in the form of refining synthetic images to make them more realistic or in the form of ``smart augmentation'', making nontrivial transformations on real data. We discuss these techniques in Section~\ref{sec:domain}. Producing synthetic data directly from random noise for classical computer vision applications generally does not sound promising: GANs can only try to approximate what is already in the data, so why can't the model itself do it?  However, in a number of applications synthetic data produced by GANs directly from random noise, usually with an abstract condition such as a segmentation mask, can help; in this section, we consider these approaches.

... Santana and Hotz~\cite{Santana2016LearningAD} present a generative model based on 
% Anders Boesen Lindbo Larsen, Søren Kaae Sønderby, Hugo Larochelle and Ole Winther, “Autoencoding beyond pixels using a learned similarity metric,” arXiv preprint arXiv:1512.09300, 2015.
that can learn to generate realistic looking images of the road for potential training of self-driving cars. ...

Counting (objects on an image) is a computer vision problem that, formally speaking, reduce to object detection or segmentation but in practice is significantly harder: to count correctly the model needs to detect all objects on the image, missing no one. Large datasets are helpful for counting, and synthetic data generated with a GAN conditioned on the number of objects or a segmentation mask with known number of objects, either produced at random or taken from a labeled real dataset, proves to be helpful. In particular, there is a line of work that deals with leaf counting on images of plants: ARIGAN by Giuffrida et al.~\cite{DBLP:journals/corr/abs-1709-00938} generates images of arabidopsis plants conditioned on the number of leaves, Zhu et al. generate the same conditioned on segmentation masks~\cite{Zhu2018DataAU}, and Kuznichov et al.~\cite{Kuznichov2019DataAF} generate synthetically augmented data that preserves the geometric structure of the leaves; all works report improved counting.

...

A related but different field considers unsupervised approaches to segmentation and other computer vision problems based on adversarial architectures, including learning to segment via cut-and-paste~\cite{Remez2018LearningTS}, unsupervised segmentation by moving objects between pairs of images with inpainting~\cite{DBLP:journals/corr/abs-1811-07630}, segmentation learned from unannotated medical images~\cite{10.1007/978-3-319-66179-7_47}, and more~\cite{Bielski2019EmergenceOO}. While this is not synthetic data \emph{per se}, in general we expect unsupervised approaches to computer vision to be an important trend in the use of synthetic data.

\subsection{Specific applications of synthetic data in computer vision}\label{sec:appl}

\subsubsection{People in CV: face recognition, person identification, pose estimation, and more}\label{sec:face}

...

There is also a related field of \emph{3D-aided face recognition}. While face recognition for full-face frontal high-quality photos has been mostly solved in 2D, achieving human and superhuman performance both for classification~\cite{6909616} and retrieval via embeddings~\cite{Schroff2015FaceNetAU}, pose-invariant face recognition \emph{in the wild}~\cite{Huang2008LabeledFI,6778340,Ding:2016:CSP:2885506.2845089}, i.e., under arbitrary angles and imperfect conditions, remains challenging. 3D-aided face recognition uses a morphable synthetic 3D model of an abstract human face that has a number of free parameters; the model learns to tune these parameters so that the 3D model fits a given photo and then uses the model and texture from the photo either to produce a frontal image or to directly recognize photos taken from other angles. This is a classic approach, dating back to late 1990s~\cite{Blanz:1999:MMS:311535.311556,1227983} and developed in many subsequent works with new morphable models~\cite{Hu2016,7350989}, deep learning used to perform the regression for morphing parameters~\cite{Tran2017RegressingRA}, extended to 3D face scans~\cite{4409029}, and so on; see, e.g., the survey~\cite{Ding:2016:CSP:2885506.2845089} for more details. Recent works used GANs to produce synthetic data for 3D-aided face recognition~\cite{Zhao2018}; we discuss this approach in detail in Section~\ref{sec:synfromreal}.

...

\cite{ijcai2018-165} \cite{DBLP:journals/corr/abs-1709-06532}

...

Wang et al.~\cite{DBLP:journals/corr/abs-1903-03303} provide a synthetic dataset GCC (see Section~\ref{sec:datapeople} for a description) for crowd counting and compare various approaches to crowd counting as a supervised problem, in particular their new spatial fully convolutional network (SFCN) model that directly predicts the density map of people on a crowded image. They report improved results when pretraining on GCC and then fine-tuning on a real dataset; they also consider GAN-based approaches that we discuss in Section~\ref{sec:damodel}. A more direct approach to generating synthetic data has been developed by Ekbatani et al.~\cite{icpram17}, who extract real pedestrians from images and add them at various locations on other backgrounds, with special improvement procedures for added realism; they also report improved counting results.

...

\todo{pose estimation} 

A very interesting application of pose estimation has been provided by Rematas et al. in a paper called ``Soccer on Your Tabletop''~\cite{8578596}. They trained specialized pose and depth estimation models for soccer players and produced a unified model that maps 2D footage of a soccer match into a 3D model suitable for rendering on a real tabletop through augmented reality devices. For training, Rematas et al. used synthetic data captured from the \emph{FIFA} video game series.

\subsubsection{Vision-based applications in unmanned aerial vehicles}\label{sec:cvnav}

A long line of research deals with vision-based approaches to operating unmanned aerial vehicles (UAV)~\cite{ALKAFF2018447}. Since in this case it is almost inevitable to use simulated environments for training, and often testing the model is also restricted to synthetic simulators (real world experiments are expensive outdoors and simply prohibited in urban environments), almost the entire field uses some kind of synthetic datasets or simulators. Classical vision-related problems for UAVs include three major tasks that UAVs often solve with computer vision:
\begin{itemize}
	\item localization and pose estimation, i.e., estimating the UAV position and orientation in both 2D (on the map) and in the 3D space; for this problem, real datasets collected by real world UAVs are available~\cite{10.1007/978-3-319-46484-8_33,Bonetto2015PrivacyIM,sensefly,Sturm2012ABF}, and the field is advanced enough to use actual field tests, so synthetic-only results are viewed with suspicion, but existing research still often employs synthetic simulators, either handmade for a specific problem~\cite{6696652} or based on professional flight simulators~\cite{DBLP:conf/fusion/AngelinoBC13};
	\item obstacle detection and avoidance, where real-world experiments are often too expensive even for testing~\cite{5152487};
	\item visual servoing, i.e., using feedback from visual sensors in order to maintain position, stability, and perform maneuvers; here synthetic data has usually been used in the form of hardware-in-the-loop simulators for the developed controllers~\cite{6224828}, sometimes augmented with full-scale flight simulators~\cite{Kurnaz:2007:ANI:1418707.1418711}.
\end{itemize}

During the latest years, these classical applications of synthetic data for UAVs have been extended and taken to new heights with modern approaches to synthetic data generation. For example, in~\cite{10.1007/978-3-030-11012-3_4} the problem is to locate safe landing areas for UAVs, which requires depth estimation and segmentation into ``horizontal'', ``vertical'', and ``uncertain'' regions to distinguish horizontal areas that would be safe for landing. To train a convolutional architecture for this segmentation and depth estimation task, the authors propose an interesting approach to generating synthetic data: they begin with Google Earth data\footnote{\url{https://www.google.com/earth/}} and extract 3D scenes from it. However, since 3D meshes in Google Earth are far from perfect, the authors then map textures to the 3D scenes to obtain less realistic-looking images but ones for which the depth maps are known perfectly. The authors show that from a bird's eye view the resulting images look quite realistic, and compare different segmentation architectures on the resulting synthetic dataset. A recent work on the same problem~\cite{Oyuki18} also compared the results obtained by training on synthetic and real datasets, with the results in favor of synthetic data due to the availability of depth maps for synthetic images.

Another interesting application where real and synthetic data come together is provided by Madaan et al.~\cite{8206190}, who solve a truly life-or-death problem for UAVs: wire detection. They use real background images and superimpose them with renderings of realistic 3D models of wires. The authors vary different properties of the wires (material, wire sag, camera angle etc.) but do not make any attempts to adapt the wires to the semantics of the background image itself, simply pasting wires onto the images. Nevertheless, Madaan et al. report good results with training first on synthetic data and then fine-tuning on a small real dataset; synthetic pretraining proves to be helpful.



\subsection{Synthetic data for character and text recognition}\label{sec:ocr}

Various tasks related to text recognition, including optical character recognition (OCR), text detection, layout analysis and text line segmentation for document digitization, and others have often been attacked with the help of synthetic data, usually with synthetic text superimposed on real images. This is a standard technique in the field because text pasted in a randomized way often looks quite reasonable even with minimal additional processing. Synthetic data was used for character detection and recognition in, e.g.,~\cite{6460871,Campos09,10.1007/978-3-642-31919-8_25,7469575} and for text block detection in, e.g.,~\cite{DBLP:journals/corr/JaderbergSVZ14,Jaderberg:2016:RTW:2877061.2877148}. Jo et al.~\cite{Jo2019} train an end-to-end convolutional architecture that can digitize documents with a mixture of handwritten and printed text; to train the network, they produce a synthetic dataset with real handwritten text superimposed on machine-printed forms, with Otsu binarization applied before pasting.

There exist published datasets of synthetic text and software to produce them, in particular MJSynth~\cite{DBLP:journals/corr/JaderbergSVZ14} and SynthText in the Wild~\cite{DBLP:journals/corr/GuptaVZ16}. In the latter work, Gupta et al. use available depth estimation and segmentation solutions to find regions (planes) of a natural image suitable for placing synthetic text and find the correct rotation of text for a given plane. Moreover, recent works have used GAN-based refinement (see Section~\ref{sec:refine}) to make synthetic text more realistic~\cite{Efimova19}. 

\subsection{Reinforcement learning in virtual environments}\label{sec:rl}

Reinforcement learning (RL) agents are commonly trained on simulations because the interactive nature of reinforcement learning makes training in the real world extremely expensive. We discuss synthetic-to-real domain adaptation in this context in Section~\ref{sec:darobot}. However, in many works, there is no explicit domain adaptation: robots are trained on simulators and later fine-tuned on real data or simply transferred to the real world. In particular, Tai et al.~\cite{8202134} learn continuous control for mapless navigation with asynchronous deep RL in virtual environments.


Computer games and game engines have been a very important source of problems and virtual environments for deep RL and AI in general~\cite{Capo2018StateOT,DBLP:journals/corr/abs-1109-1314,8632747}. Much of the foundational work in modern deep RL has been done in the environments of 2D arcade games, usually classical \emph{Atari} games~\cite{Bellemare:2013:ALE:2566972.2566979,mnih2015humanlevel}. 
% Works on robotic navigation use synthetic simulators extensively. 
First, many new ideas for RL architectures or training procedures for robotic navigation were introduced as direct applications of deep RL to navigation in complex synthetic environments, in particular to navigating mazes in video games such as \emph{Doom}~\cite{DBLP:journals/corr/BhattiDMNST16} and \emph{Minecraft}~\cite{Oh:2016:CMA:3045390.3045684} or specially constructed 3D mazes, e.g., from the \emph{DeepMind Lab} environment~\cite{DBLP:journals/corr/BeattieLTWWKLGV16,8460646}. \emph{Doom} became something of an industry standard, with the \emph{VizDoom} framework developed by Kempka et al.~\cite{DBLP:journals/corr/KempkaWRTJ16} and later used in many important works~\cite{Alvernaz2017AutoencoderaugmentedNF,Ratcliffe2017ClydeAD,Lample:2017:PFG:3298483.3298548,Wu2017TrainingAF}. Games of other genres, in particular real-time strategy games~\cite{8490409,Tang2018ARO}, also represent a rich source of synthetic environments for deep RL; we note the \emph{TorchCraft} library for machine learning research in \emph{StarCraft}~\cite{DBLP:journals/corr/SynnaeveNACLLRU16}, synthetic datasets extracted from \emph{StarCraft}~\cite{DBLP:journals/corr/abs-1708-02139,DBLP:journals/corr/abs-1712-10179,Wu2017MSCAD}, the \emph{ELF} (Extensive, Lightweight, and Flexible) library platform with three simplified real-time strategy games~\cite{DBLP:journals/corr/TianGSWZ17}, and the SC2LE (StarCraft II Learning Environment) library for \emph{Starcraft II}~\cite{DBLP:journals/corr/abs-1708-04782}. Racing games have been used as environments for training end-to-end RL driving agents~\cite{8014798}. While data from computer games could technically be considered synthetic data, we do not go into further details on game-related research and concentrate on virtual environments specially designed for machine learning and/or transfer to real world tasks. Note, however, that synthetic data is already making inroads even into learning to play computer games: Justesen et al.~\cite{DBLP:journals/corr/abs-1806-10729} show that using procedurally generated levels improves generalization and final results for \emph{Atari} games and can even produce models that work well when evaluated on a completely new level every time they play.

Sadeghi and Levine~\cite{Sadeghi2017CAD2RLRS} present the $\mathrm{CAD}^2\mathrm{RL}$ framework for avoiding collisions while flying in indoor environments. They motivate the use of synthetic data by the domain randomization idea (see also Section~\ref{sec:domrand}) and produce a wide variety of indoor simulated environments constructed in \emph{Blender}. They do not use any real images during training, learning the Q-function for the reinforcement learning agent entirely on simulated data, with a fully convolutional neural network. The authors report improvements in a number of complex settings such as flying around corners, navigating through narrow corridors, flying up a staircase, avoiding dynamic obstacles, and so on.

Robotics \cite{Bayraktar2018AHI}

~\cite{}. 

Using physics simulators as synthetic environments:
\cite{Pecka2018DataDrivenPT}

\subsubsection{Synthetic data for autonomous driving}

Autonomous driving survey~\cite{machines5010006}

\cite{Yue2018ALP} 

The original paper on the CARLA simulator~\cite{Dosovitskiy17} also provides a comparison on synthetic data between conditional imitation learning, deep reinforcement learning, and a modular pipeline with separated perception, local planning, and continuous control, with limited success but generally best results obtained by the modular pipeline. 

...

Many works on autonomous driving use TORCS~\cite{TORCS} (see Section~\ref{sec:dataoutdoor}) as a testbed, both in virtual autonomous driving competitions and simply as a well-established research platform. We do not aim to provide a full in-depth survey of the entire field and only note that despite its long history TORCS is being actively used for research purposes up to this day. In particular, Sallab et al.~\cite{Sallab2016EndtoEndDR,Sallab2017DeepRL} use it in their deep reinforcement learning frameworks for lane keeping assist and autonomous driving, Xiong et al.~\cite{DBLP:journals/corr/XiongWZL16} add safety-based control on top of deep RL, Wang et al.~\cite{DBLP:journals/corr/abs-1811-11329} train a deep RL agent for autonomous driving in TORCS, Barati et al.~\cite{DBLP:journals/corr/abs-1905-03985} use it to add multi-view inputs for deep RL agents, Li et al.~\cite{DBLP:journals/corr/abs-1810-12778} develop \emph{Visual TORCS}, a deep RL environment based on TORCS, Ando, Lubashevsky et al.~\cite{2015arXiv151104640A,2016arXiv160901812L} use TORCS to study the statistical properties of human driving, Glassner et al.~\cite{DBLP:journals/corr/abs-1901-00114} shift the emphasis to trajectory learning, Luo et al.~\cite{DBLP:journals/corr/abs-1811-06151} use TORCS as the main test environment for a new variation of the policy gradient algorithm, Liu et al.~\cite{DBLP:journals/corr/LiuSPVK17} make use of the multimodal sensors available in TORCS for end-to-end learning, Xu et al.~\cite{DBLP:journals/corr/abs-1801-05299} train a segmentation network and feed segmentation results to the RL agent in order to unify synthetic imagery from TORCS and real data, and so on. In an interesting recent work, Choi et al.~\cite{DBLP:journals/corr/abs-1809-01822} consider the driving experience transfer problem but consider it not from a synthetic simulator to the real domain but from one simulator (TORCS) to another (GTA V).


\subsection{Synthetic data in natural language processing}\label{sec:nlp}

Synthetic data has not been widely used in natural language processing (NLP). In our opinion, there is a conceptual reason for this. Compare with computer vision: there, the process of synthetic data generation can be done separately from learning the models, and the essence of what the models are learning is, in a way, ``orthogonal'' to the difference between real and synthetic data. If I show you a cartoon add featuring a new bottle of soda, you will be able to find it in a supermarket even though you would never confuse the cartoon with a real photo. In natural language processing, on the other hand, text generation is the hard problem itself. The problem of generating meaningful synthetic text with predefined target variables such as topic or sentiment is the subject of many studies in NLP, we are still a long way to go before it is solved, and it is quite probable that when it finally is solved, discriminative models for the target variables will easily follow from it, rendering synthetic data useless.

Nevertheless, there have been works that use data augmentation for NLP in a fashion that borders on using synthetic data. There have been simple augmentation approaches such as to simply drop out certain words~\cite{W16-2323}. A development of this idea shown in~\cite{D18-1100} switches out certain words, replacing them 
% neither with zeros (as dropout does) nor with synonyms but 
with random words from the vocabulary. The work~\cite{Xie2017DataNA} develops methods of data noising for language models, adding noise to word counts in a way reminiscent of smoothing in language models based on $n$-grams.

A more developed approach is to do data augmentation with synonyms: to expand a dataset, one can replace words with their synonyms, getting ``synthetic sentences'' that can still preserve target variables such as the topic of the text, its sentiment, and so on. The work~\cite{NIPS2015_5782} used this method directly to train a character-level network for text classification, while~\cite{GAN16} tested augmentation with synonyms for morphology-rich languages such as Russian. In~\cite{P17-2090}, augmentation with synonyms was used for low-resource machine translation, with an auxiliary LSTM-based language model used to recognize whether the synonym substitution is correct. The work~\cite{Wang2015ThatsSA}, which concentrated on studying tweets, proposed to use embedding-based data augmentation, using neighboring words in the word vector space as synonyms. The work~\cite{N18-2072} extends augmentation with synonyms by replacing words in sentences with other words in paradigmatic relations with the original words, as predicted by a bi-directional language model at the word positions. 

...


\subsection{Synthetic data for neural programming}\label{sec:other}

Another interesting domain where synthetic data is paramount is neural program synthesis and neural program induction. The basic idea of teaching a machine learning model to program can be broadly divided into two subfields: program induction aims to train an end-to-end differentiable model to capture an algorithm~\cite{NIPS2017_6803}, while program synthesis tries to teach a model the semantics of a domain-specific language (DSL), so that the model is able to generate programs according to given specifications~\cite{DBLP:journals/corr/abs-1802-02353}. Basically, in program induction the network \emph{is} the program, while in program synthesis the network \emph{writes} the program. Naturally, both tasks require large datasets of programs together with their input-output pairs; since no such large datasets exist, and generating synthetic programs and running them in this case is relatively easy (arguably even easier than generating synthetic data for computer vision), all modern works use synthetic data to train the ``neural computers''.

\begin{figure}[!t]\centering
% \begin{tabular}{p{.45\linewidth}p{.45\linewidth}}
\begin{minipage}[b]{.36\linewidth}
\textbf{Input}:
\begin{verbatim}
j=8584
for x in range(8):
    j+=920
b=(1500+j)
print((b+7567))
\end{verbatim}
\textbf{Target}: \verb$25011$.
\end{minipage}
~
\begin{minipage}[b]{.6\linewidth}
\textbf{Input}:
\begin{verbatim}
i=8827
c=(i-5347)
print((c+8704) if 2641<8500 else 5308)
\end{verbatim}
\textbf{Target}: \verb$12184$.
\end{minipage}
% \end{tabular}

\caption{Sample synthetic programs from~\cite{DBLP:journals/corr/ZarembaS14}.}\label{fig:prog}
\end{figure}

In program induction, the tasks are so far relatively simple, and synthetic data generation does not present too many difficulties. For example, Joulin and Mikolov~\cite{Joulin:2015:IAP:2969239.2969261} present a new architecture (stack-augmented recurrent networks) to learn regularities in algorithmically generated sequences of symbols; the training data, as in previous such works~\cite{10.1007/3540634932_25,Hochreiter:1997:LSM:1246443.1246450,Wiles1995LearningTC,963769}, is synthetically generated by hand-crafted simple algorithms, including generating sequences from a pattern such as $a^nb^{2n}$ or $a^nb^mc^{n+m}$, binary addition (supervised problem asking to continue a string such as $110+10=$), and similar.  Zaremba and Sutskever~\cite{DBLP:journals/corr/ZarembaS14} train a model to execute programs, i.e., map their textual representations to outputs; they generate training data as Python-style programs with addition, subtraction, multiplication, variable assignments, if-statements, and for-loops (but without nested loops), each ending with a \texttt{print} statement; see Fig.~\ref{fig:prog} for an illustration. Neural RAM machines~\cite{45398} are trained on a number of simple tasks (access, increment, copy etc.) whose specific instances are randomly synthesized. The same goes for neural Turing machines~\cite{DBLP:journals/corr/GravesWD14} and neural GPUs~\cite{Kaiser2016NeuralGL,Freivalds2017ImprovingTN}: they are trained and evaluated on synthetic examples generated for simple basic problems such as copying, sorting, or arithmetic operations.

In neural program synthesis, again, the programs are usually simple and also generated automatically; attempts to collect natural datasets for program synthesis have begun only very recently~\cite{DBLP:journals/corr/abs-1807-03168}. Learning-based program synthesis (earlier attempts were based on logical inference~\cite{Manna:1971:TAP:362566.362568}) began with learning string manipulation programs~\cite{Gulwani:2011:ASP:1925844.1926423} and soon branched into deep learning, using recurrent architectures to guide search-based methods~\cite{DBLP:journals/corr/abs-1804-01186} or to generate programs in encoder-decoder architectures~\cite{DBLP:journals/corr/DevlinUBSMK17,chen2019}. In~\cite{DBLP:journals/corr/abs-1805-04276,si2019}, reinforcement learning is added on top of a recurrent architecture in order to alleviate the \emph{program aliasing} problem, i.e., the fact that many different equivalent programs provide equally correct answers while the training set contains only one. All of the above-mentioned models were trained on synthetic datasets of randomly generated programs (usually in the form of abstract syntax trees) run on randomized sets of inputs.

As a separate thread, we mention works on program synthesis for visual reasoning and, generally speaking, question answering~\cite{Johnson2017,Santoro2017ASN,DBLP:journals/corr/HuARDS17}. To do visual question answering~\cite{Agrawal2017}, models are trained to compose a short program based on the natural language question that will lead to the answer, usually in the form of an execution graph or a network architecture. This line of work is based on neural module networks~\cite{DBLP:journals/corr/AndreasRDK15,DBLP:journals/corr/abs-1809-08697} and similar constructions~\cite{DBLP:journals/corr/HuRADS16,DBLP:journals/corr/AndreasRDK16}, where the network learns to create a composition of modules (in QA, based on parsing the question) that are also neural networks, all learned jointly (see, however, the critique in~\cite{SEJNOVA2018481}). Latest works use architectures based on self-attention that have proven their worth across a wide variety of NLP tasks~\cite{lewis2018generative}. Naturally, most of these works use the CLEVR synthetic dataset for evaluation (see Section~\ref{sec:datareason}).

Generation of synthetic data itself has not been given much attention in this field until very recently, but the interest is rising. The work by Shin et al.~\cite{shin2018synthetic} presents a study of contemporary synthetic data generation techniques for neural program synthesis and concludes that the resulting models do not capture the full semantics of the language, even if they do well on the test set. Shin et al. show that synthetic data generation algorithms, including the one from the popular \emph{tensor2tensor} library~\cite{tensor2tensor}, have biases that fail to cover important parts of the program space and deteriorate the final result. To fix this problem, they propose a novel methodology for generating distributions over the space of datasets for program induction and synthesis, showing significant improvements for two important domains: Calculator (which computes the results of arithmetic expressions) and Karel (which achieves a given objective with a virtual robot moving on a two-dimensional grid with walls and markers). We expect more research into synthetic data generation for neural program induction and synthesis to follow in the near future.

\subsection{Synthetic data in bioinformatics}\label{sec:bio}

We use examples from the heathcare and biomedical domain throughout this survey; see, e.g., Sections~\ref{sec:medical} and~\ref{sec:finance}. In this section, we concentrate on applications of synthetic data in bioinformatics that fall outside either producing synthetic medical images (usually through GANs, see Section~\ref{sec:medical}) or providing privacy guarantees for sensitive data through synthetic datasets (Section~\ref{sec:finance}). It turns out that there are still plenty, and synthetic data is routinely used and generated throughout bioinformatics; see also a survey in~\cite{doi:10.1098/rsif.2017.0387}.

For many of these methods, generated synthetic data is the end goal rather than a tool to improve machine learning models. In particular, \emph{de novo} drug design~\cite{doi:10.1021/acs.jmedchem.5b01849,doi:10.1002/wcms.49} is a field that searches for molecules with desirable properties in a search space of about $10^{60}$ synthesizable molecules~\cite{ChEMBL,doi:10.1002/wcms.1104}, and the goal is to find (which in a space of this size rather means to \emph{generate}) candidate molecules that would later have to be explored further in lab studies and then clinical trials. First modern attempts at \emph{de novo} drug design used rule-based methods that simulate chemical reactions~\cite{doi:10.1021/acs.jmedchem.5b01849}, but the field soon turned to generative models, in particular based on deep learning~\cite{Gawehn15,CHEN20181241}. In this context, molecules are usually represented in the SMILES format~\cite{doi:10.1021/ci00057a005} that encodes molecular graphs as strings in a certain formal grammar, which makes it possible to use sequence learning models to generate new SMILES strings. Segler et al.~\cite{DBLP:journals/corr/SeglerKTW17} used LSTM-based RNNs to learn a chemical language model, while G{\'o}mez-Bombarelli et al.~\cite{DBLP:journals/corr/Gomez-Bombarelli16} trained a variational autoencoder (VAE) which is already a generative model capable of generating new candidate molecules. To further improve generation, Kusner et al.~\cite{2017arXiv170301925K} developed a novel extension of VAEs called Grammar Variational Autoencoders that can take into account the rules of the SMILES formal grammar and make VAE outputs conform to the grammar. To then use the models to obtain molecules with desired properties, researchers used either a small set of labeled positive examples~\cite{DBLP:journals/corr/SeglerKTW17} or augment the RNN training procedure with reinforcement learning~\cite{DBLP:journals/corr/JaquesGTE16}. In particular, Olivecrona et al.~\cite{Olivecrona2017} use a recurrent neural network trained to generate SMILES representations: first, a prior network (3 layers of 1024 GRU) is trained in a supervised way on the RDKit subset~\cite{Landrum2016RDKit2016_09_4} of ChEMBL database~\cite{ChEMBL}, then an RL agent (with the same structure, initialized from the prior network) is fine-tuned with the REINFORCE algorithm to improve the resulting SMILES encoding. A similar architecture, but with a stack-augmented RNN~\cite{DBLP:journals/corr/JoulinM15} as the basis, which enables more long-term dependencies, was presented by Popova et al.~\cite{Popovaeaap7885}. We note a series of works by \emph{Insilico} researchers Kadurin, Polykovskiy and others who applied different generative models to this problem:
\begin{itemize}
	\item the work~\cite{Kadurin16} trains a supervised adversarial autoencoder~\cite{44904} with the condition (in this case, growth inhibition percentage for tumor cells after treatment) added as a separate neuron to the latent layer;
	\item in~\cite{KNKAZ17}, Kadurin et al. compared adversarial autoencoders (AAE) with variational autoencoders (VAE) for the same problem, with new modifications to the architecture that result in improved generation;
	\item in~\cite{doi:10.1021/acs.molpharmaceut.8b00839}, Polykovskiy et al. introduced a new AAE modification, entangled conditional adversarial autoencoder, to ensure the disentanglement of latent features; in this case, which is still quite rare for deep learning in drug discovery, a newly discovered molecule (a new inhibitor of Janus kinase 3) was actually tested in the lab and showed good activity and selectivity \emph{in vitro};
	\item Kuzmynikh et al.~\cite{KPKZBNSZ18} presented a novel 3D molecular representation based on the wave transform that led to improved performance for CNN-based autoencoders and improved MACCS fingerprint prediction;
	\item Polykovskiy et al.~\cite{PZSGTBKAAVKNAZ18} presented MOSES (Molecular Sets), a benchmarking platform for molecular generation models, which implemented and compared various generative models for molecular generation including CharRNN~\cite{doi:10.1021/acscentsci.7b00512}, VAE, AAE, and Junction Tree VAE~\cite{2018arXiv180204364J}, together with a variety of evaluation metrics for generation results.
\end{itemize}
The above works can be thought of as generation of synthetic data (e.g., molecular structures) that could be of direct use for practical applications.

Johnson et al.~\cite{2017arXiv170500092J} undertake an ambitious project: they learn a generative model of the variation in cell and nuclear morphology based on fluorescence microscopy images. Their model is based on two adversarial autoencoders~\cite{44904}, one learning a probabilistic model of cell and nuclear shape and the other learning the interrelations between subcellular structures conditional on an encoding of the cell and nuclear shape from the first autoencoder. The resulting model produces plausible synthetic images of the cell with known localizations of subcellular structures.

One interesting variation of ``synthetic data'' in bioinformatics concerns learning from live experiments on synthetically generated biological material. For example, Rosenberg et al.~\cite{ROSENBERG2015698} study alternative RNA splicing, in particular the functional effects of genetic variation on the molecular phenotypes through alternative splicing. To do that, they create a large-scale gene library with more than two million randomly generated synthetic DNA sequences, then used massively parallel reporter assays (MPRA) to measure the isoform ratio for all mini-genes in the experiment, and then used it to learn a (simple linear) machine learning model for alternative splicing. It turned out that this approach significantly improved prediction quality, outperforming state of the art deep learning models for alternative splicing trained on the actual human genome~\cite{Xiong1254806} in predicting the results of \emph{in vivo} experiments. There is also a related field of imitational modeling for bioinformatics data that often results in realistic synthetic generators; e.g., Van den Bulcke et al.~\cite{VandenBulcke2006} provide a generator for synthetic gene expression data, able to produce synthetic transcriptional regulatory networks and simulated gene expression data while closely matching real statistics of biological networks.




==> datasets.tex <==
\section{Synthetic datasets}\label{sec:datasets}

In this section, we present an overview of popular synthetic datasets that have been widely used in recent studies. We organize this section by classifying datasets with respect to use cases, from generic object detection and segmentation problems to specific domains such as aerial simulators. All of these domains benefit highly from pixel-perfect labeling available by default in synthetic data, both in the form of classical computer vision labeling---bounding boxes for objects, segmentation masks---and labeling that would be very hard or impossible to do by hand: depth estimation, stereo image matching, 3D labeling in voxel space and so on.

We also note that while collecting synthetic datasets is a challenging task by itself, it is insufficient to train, e.g., an autonomous vehicle such as a self-driving car or a drone, or an industrial robot. Learning to control a vehicle or robot often requires \emph{reinforcement learning}, where an agent has to learn from interacting with the environment, and real world experiments to train a self-driving car or a robotic arm are completely impractical. Fortunately, this is another field where synthetic data shines: once one has a fully developed 3D environment that can produce datasets for computer vision or other sensory readings, it is only one more step to active interaction with this environment. Again, techniques based on or developed for computer games are extremely helpful, since games are developed with real-time interaction in mind. Therefore, in most domains considered below we can see the shift from static synthetic datasets to interactive simulation environments.

% \subsection{Basic computer vision problems in 2D and 3D}\label{sec:datavis}

\subsection{Low-level computer vision problems}\label{sec:datalow}

Low-level computer vision problems include, in particular, \emph{optical flow estimation}, i.e., estimating the distribution of apparent velocities of movement along the image, \emph{stereo image matching}, i.e., finding the correspondence between the points of two images of the same scene from different viewpoints, \emph{background subtraction}, and so on. Algorithms for solving these problems can serve as the foundation for computer vision systems, e.g., optical flow is important for motion estimation and video compression. Low-level problems can usually be approached with methods that do not require modern large-scale datasets or much learning at all, e.g., classical differential methods for optical flow estimation. However, at the same time, ground truth datasets are very hard to label manually, and hardware sensors that would provide direct measurements of optical flow or stereo image correspondence are difficult to construct (e.g., commodity optical flow sensors simply run the same estimation algorithms).

All of these reasons make low-level computer vision one of the oldest problems where synthetic data was successfully used, originally mostly for evaluation. Works as far back as late 1980s~\cite{47107} and early 1990s~\cite{Barron1994} presented and used synthetic datasets to evaluate different optical flow estimation algorithms. In 1999, Freeman et al.~\cite{790414} presented a synthetically generated world of images labeled from their 3D scenes designed to train and evaluate low-level computer vision algorithms.

A modern dataset for low-level vision is \emph{Middlebury} presented by Baker et al.~\cite{Baker2011}; in addition to ground truth real life measurements taken with specially constructed computer-controlled lighting, they provide realistic synthetic imagery as part of the dataset and include it in the large-scale evaluation of optical flow and stereo correspondence estimation algorithms that they undertake. The \emph{Middlebury} dataset played an important role in the development of low-level computer vision algorithms~\cite{988771,Seitz:2006:CEM:1153170.1153518}, but its main emphasis was still on real imagery, as evidenced by its next version, \emph{Middlebury 2014}~\cite{conf/dagm/ScharsteinHKKNWW14}.

Butler et al.~\cite{10.1007/978-3-642-33783-3_44} presented a synthetic optical flow dataset \emph{MPI-Sintel} derived from the short animated movie Sintel\footnote{\url{http://www.sintel.org/}} produced as part of the Durian Open Movie Project. The main characteristic feature of \emph{MPI-Sintel} is that it contains the same scenes with different render settings, with different quality and complexity, which can provide a deeper understanding of where different optical flow algorithms break down. This is an interesting idea that has not yet found its way into synthetic data for deep learning-based computer vision but might be worthwhile to investigate.

As the field moved from classical unsupervised approaches to deep learning, state of the art models began to require large datasets that could not be produced in real life, and after the transition to deep learning synthetic datasets started to dominate. Dosovitsky et al.~\cite{7410673} presented a large synthetic dataset called \emph{Flying Chairs} from a public database of 3D chair models, adding them on top of real backgrounds to train a CNN-based optical flow estimation model. Mayer et al.~\cite{DBLP:journals/corr/MayerIHFCDB15} extended this work from optical flow to disparity and scene flow estimation, presenting three synthetic datasets produced in Blender (similar to Sintel): \emph{FlyingThings3D} with everyday objects flying along randomized trajectories, \emph{Monkaa} from its namesake animated short film with soft nonrigid motion and complex details such as fur, and \emph{Driving} with naturalistic dynamic outdoor scenes from the viewpoint of a driving car (for more outdoor datasets see Section~\ref{sec:dataoutdoor}). The \emph{UnrealStereo} dataset by Zhang et al.~\cite{Zhang2016UnrealStereoAS} is a stereo scene analysis dataset based on the \emph{Unreal Engine 4} designed to evaluate the robustness of stereo vision algorithms to changes in material and other scene parameters. Many datasets that we describe below for high-level problems, such as SceneNet RGB-D~\cite{8237554} or SYNTHIA~\cite{7780721}, also contain the labeling for optical flow and have been used to train the corresponding models.

In a recent work, Mayer et al.~\cite{Mayer:2018:MGS:3270334.3270407} provide an overview of different synthetic datasets for low-level computer vision and compare them from the standpoint of training optical flow models. They come to interesting conclusions:
\begin{itemize}
	\item first, for low-level vision synthetic data does not have to be realistic, \emph{Flying Chairs} works just fine; 
	\item second, it is best to combine different synthetic datasets and train in a variety of situations and domains; this ties into the domain randomization idea that we discuss in Section~\ref{sec:domrand};
	\item third, while realism itself is not needed, it does help to simulate the flaws of a specific real camera; Mayer et al. show that simulating, e.g., lens distortion and blur or Bayer interpolation artifacts in synthetic data improves the results on the test set afterwards.
\end{itemize}
The question of realism remains open for synthetic data, and we will touch upon it many times in the survey. While it does seem plausible that for low-level problems such as optical flow estimation ``low-level realism'' (simulating camera idiosyncrasies) is much more important than high-level scene realism, the answer may be different for other problems.

\subsection{Basic high-level computer vision}\label{sec:datahigh}

% \subsubsection{Object recognition and segmentation}

The basic high-level computer vision problems, object detection and segmentation, fully enjoy the benefits of perfect labeling provided by synthetic data, and there is plenty of effort devoted to making synthetic data work for these problems. Since making synthetic data requires the development of 3D models, datasets usually also feature labeling related to 3D such as the depth map, labeled 3D parts of a shape, volumetric 3D data, and so on.

Many works apply synthetic data to recognizing everyday objects such as, e.g., retail items, food, or furniture, and most of them draw upon the same database for 3D models. Developed by Chang et al.~\cite{DBLP:journals/corr/ChangFGHHLSSSSX15}, ShapeNet\footnote{\url{https://www.shapenet.org/}} indexes more than three million models, with $220{,}000$ of them classified into $3{,}135$ categories that match WordNet synsets. Apart from the class labels, ShapeNet also includes geometric, functional, and physical annotations, including planes of symmetry, part hierarchies, weight and materials, and more. Researchers often use the clean and manually verified ShapeNetCore subset that covers $55$ common object categories with about $51{,}000$ unique 3D models~\cite{DBLP:journals/corr/abs-1710-06104}. 

ShapeNet has become the basis for further efforts devoted to improving labelings. In particular, region annotation (e.g., breaking an airplane into wings, body, and tail) is a manual process even in a synthetic dataset, while shape segmentation models increasingly rely on synthetic data~\cite{Yi:2017:LHS:3072959.3073652}; this also relates to the 3D mesh segmentation problem~\cite{doi:10.1111/j.1467-8659.2007.01103.x}. Based on ShapeNet, Yi et al.~\cite{Yi:2016:SAF:2980179.2980238} developed a framework for scalable region annotation in 3D models based on active learning, and Chen et al.~\cite{Chen:2009:BMS:1531326.1531379} released a benchmark dataset for 3D mesh segmentation. A recent important effort related to ShapeNet is the release of PartNet~\cite{DBLP:journals/corr/abs-1812-02713}, a large-scale dataset of 3D objects annotated with fine-grained, instance-level, and hierarchical 3D part information; it contains $573{,}585$ part instances across $26{,}671$ 3D models from $24$ object categories. PartNet is mostly intended as a benchmark for 3D object and scene understanding, but the corresponding 3D models will no doubt be widely used to generate synthetic data.

One common approach to generating synthetic data is to reuse the work of 3D artists that went into creating the virtual environments of video games. For example, Richter et al.~\cite{DBLP:journals/corr/abs-1709-07322,DBLP:journals/corr/RichterVRK16} captured datasets from the Grand Theft Auto V video game (see also Section~\ref{sec:dataoutdoor}). They concentrated on semantic segmentation; note that getting pixel-wise labels for segmentation still required manual labor, but the authors claim that by capturing the communication between the game and the graphics hardware, they have been able to cut the labeling costs (in annotation time) by orders of magnitude. Once the annotator has worked through the first frame, the same combinations of meshes, textures, and shaders reused on subsequent frames can be automatically recognized and labeled, and the annotators are only asked to label new combinations. In essence, the game engine provides perfect superpixels that are persistent across frames.

As \emph{Grand Theft Auto V} and other games became popular for collecting synthetic datasets (see also Section~\ref{sec:dataoutdoor}), more specialized solutions began to appear. One such solution is \emph{UnrealCV} developed by Qiu et al.~\cite{DBLP:journals/corr/QiuY16,qiu2017unrealcv}. This is an open-source plugin for the popular game engine \emph{Unreal Engine 4} that provides commands that allow to get and set camera location and field of view, get the set of objects in the scene with their positions, set lighting parameters, modify properties of the objects such as material, and capture from the engine the image and depth ground truth for the current camera and lighting parameters. This allows to create synthetic image datasets from realistic virtual worlds.

Robotics has motivated the appearance of synthetic datasets with objects that might be subject for manipulation, usually with fairly accurate models of their physical properties. The computer vision objectives in these datasets usually relate to robotic perception and include segmentation, depth estimation, object pose estimation, and object tracking. In particular, Choi et al.~\cite{6696485} presented a dataset of 3D models of household objects for their tracking filter, while Hodan et al.~\cite{DBLP:journals/corr/HodanHOMLZ17} provide a real dataset of textureless objects supplemented with 3D models of these objects that provide the 6D ground truth poses. The Yale-CMU-Berkeley (YCB) Object and Model set presented by Calli et al.~\cite{7251504} contains a set of 3D models of objects commonly used for robotic grasping together with a database of real RGB-D scans and physical properties of the objects, which makes it possible to use them in simulations. The \emph{Falling Things} (FAT) dataset by NVIDIA researchers Tremblay et al.~\cite{8575443} contains about 61500 images of 21 household objects taken from the YCB dataset and placed into virtual environments under a wide variety of lighting conditions, with 3D poses, pixel-perfect segmentation, depth images, and 2D/3D bounding box coordinates for each object. 

...

Abu Alhaija et al.~\cite{AbuAlhaija2018} and Georgakis et al.~\cite{Georgakis2017SynthesizingTD} propose procedures to augment real backgrounds with synthetic objects (see also Section~\ref{sec:cutpaste} where we discuss placing real objects on real backgrounds). In~\cite{AbuAlhaija2018}, the backgrounds come from the KITTI dataset of outdoor scenes and the objects are synthetic models of cars, while in~\cite{Georgakis2017SynthesizingTD} the authors place synthetic objects into indoor scenes with an eye towards home service robots. Synthetic objects have been used on real backgrounds many times before, but the main distinguishing feature of~\cite{AbuAlhaija2018} and~\cite{Georgakis2017SynthesizingTD} is that they are able to paste synthetic objects on real surfaces in a way consistent with the rest of the background scene. Abu Alhaija et al. developed a pipeline for automated analysis that recognized road surfaces on 360\textdegree, but at the same time they conclude that the best (w.r.t. to the quality of the resulting segmentation model) way to insert the cars was to do it manually, and almost all their experiments used manual car placement. These experiments showed that state of the art models for instance segmentation and object detection yield better results on real validation tests when trained on scenes augmented with synthetic cars. Georgakis et al. use the algorithm from~\cite{Taylor2012ParsingIS} to extract supporting surfaces from an image and place synthetic objects on such surfaces with proper scale; they show significant improvements by training on hybrid real+synthetic datasets.

% \subsection{Depth estimation, stereo images, [MORE]}


Underwater \cite{Olson2018SyntheticDG}...

\subsection{Synthetic people}\label{sec:datapeople}


...Bak et al.~\cite{Bak2018DomainAT} present the \emph{Synthetic Data for person Re-Identification} (SyRI) dataset with virtual 3D humans designed with \emph{Adobe Fuse CC} to make the models and \emph{Unreal Engine 4} for high-speed rendering. Interestingly, they model realistic lighting conditions by using real HDR environment maps collected with light probes and panoramic photos.

Another important application of datasets of synthetic people is crowd counting. In this case, collecting ground truth labels, especially if the model is supposed to do segmentation in addition to simple counting, is especially labor-intensive since crowd counting scenes are often highly congested and contain hundreds of people. Existing real datasets are either relatively small or insufficiently diverse; e.g., the UCSD dataset~\cite{4587569} and the Mall dataset~\cite{Chen2012FeatureMF} have both about 50{,}000 pedestrians but in each case collected from a single surveillance camera, the ShanghaiTech dataset~\cite{7780439} has about 330{,}000 heads but only about 1200 images, again collected on the same event, and the UCF-QNRF dataset~\cite{DBLP:journals/corr/abs-1808-01050}, while more diverse than previous ones, is limited to extremely congested scenes, with up to 12{,}000 people on the same image, and has only about 1500 images. To provide sufficient diversity and scale, Wang et al.~\cite{DBLP:journals/corr/abs-1903-03303} presented a synthetic dataset collected with the help of the Grand Theft Auto V engine; the released dataset contains about 15{,}000 synthetic images with more than 7{,}5 million annotated people in a wide variety of scenes.


\subsection{Outdoor scenes and navigation}\label{sec:dataoutdoor}

An important direction of applications for synthetic data is related to navigation, localization and mapping (SLAM), or similar problems intended to improve the motion of autonomous robots. Possible applications include SLAM, motion planning, and motion for control for self-driving cars (urban navigation) CITE, unmanned aerial vehicles~\cite{KanellakisN17,ALKAFF2018447,COURBON2010789}, and more; see also general surveys of computer vision for mobile robot navigation~\cite{982903,Bonin-Font2008}.

Before proceeding to current state of the art, we note an interesting historical fact: one of the first autonomous driving attempts based on neural networks, ALVINN~\cite{Pomerleau:1989:AAL:89851.89891}, which used as input $30\times 32$ videos supplemented with $8\times 32$ range finder data, was already training on synthetic data. As early as 1989, the authors remark that ``training on actual road images is logistically difficult because... the network must be presented with a large number of training exemplars... under a wide variety of conditions'' and proceed to describing a simulator. One of the first widely adopted full-scale visual simulation environments for robotics, \emph{Gazebo} by Koenig and Howard~\cite{1389727}, provided both indoor and outdoor environment for robotic control training.

% ...

In a much more recent effort, Xerox researchers Gaidon et al.~\cite{Gaidon:Virtual:CVPR2016} presented a photo-realistic synthetic video dataset Virtual KITTI\footnote{The name comes from the KITTI dataset~\cite{Geiger2013IJRR,Menze2015CVPR} created in a joint project of the Karlsuhe Institute of Technology and Toyota Technological Institute at Chicago.} intended for object detection and multi-object tracking, scene-level and instance-level semantic segmentation, optical flow, and depth estimation. The dataset contains five different virtual outdoor environments created with the Unity game engine and 50 photo-realistic synthetic videos. Gaidon et al. studied existing multi-object trackers, e.g., based on an improved min-cost flow algorithm~\cite{5995604} and on Markov decision processes~\cite{7410891}; they found minimal real-to-virtual gap. Note, however, that experiments in~\cite{Gaidon:Virtual:CVPR2016} were done on trackers trained on real data evaluated on the synthetic videos (and that's where they worked well), not the other way around. In general, the Virtual KITTI dataset is much too small to train a model on it, it is intended for evaluation, which also explains the experimental setup.

Johnson-Robertson et al.~\cite{7989092}, on the other hand, presented a method to \emph{train} on synthetic data. They collected a large dataset by capturing scene information from the \emph{Grand Theft Auto V} video game that provides top-of-the-line graphics and at the same time stores scene information such as depth maps and rough bounding boxes in the GPU stencil buffer, which can also be captured; the authors developed an automated pipeline to obtain tight bounding boxes. Three datasets were generated, with 10K, 50K, and 200K images respectively. The main positive result of~\cite{7989092} is that a standard Faster R-CNN architecture~\cite{7485869} trained on 50K and 200K images outperformed on a real validation set (KITTI) the same architecture trained on a real dataset. The real training set was \emph{Cityscapes}~\cite{Cordts2016Cityscapes} that contains 2{,}975 images, so while the authors used more synthetic data than real, the difference is only 1-2 orders of magnitude. The datasets by Richter et al.~\cite{DBLP:journals/corr/abs-1709-07322,DBLP:journals/corr/RichterVRK16} were also captured from \emph{Grand Theft Auto V} 

The SYNTHIA dataset presented by Ros et al.~\cite{7780721} provides synthetic images of urban scenes labeled for semantic segmentation. It consists of renderings of a virtual city constructed with the Unity platform by the authors and includes segmentation annotations for 13 classes such as pedestrians, cyclists, buildings, roads, and so on. The dataset contains more than $213{,}000$ synthetic images covering a wide variety of scenes and environmental conditions; experiments in~\cite{7780721} show that augmenting real datasets with SYNTHIA leads to improved segmentation.

Tian et al.~\cite{Tian18} present the \emph{ParallelEye} synthetic dataset for urban outdoor scenes. Their approach is rather flexible and relies on previously developed \emph{Esri CityEngine} framework~\cite{6737786} that provides capabilities for batch generation of 3D city scenes based on terrain data. In~\cite{Tian18}, this data is automatically extracted from the OpenStreetMap platform\footnote{\url{https://www.openstreetmap.org/}}. The 3D scene is then imported into the Unity3D game engine, which helped add urban vehicles on the roads, set up traffic rules, add support for different weather and lighting conditions. Tian et al. showed improvements in object detection quality for state of the art architectures trained on \emph{ParallelEye} and tested on the real KITTI test set as compared to training on the real KITTI training set.

AADS \cite{Li2019AADSAA}

Aerial simulation~\cite{Bondi2018AirSimWAS}

Synthetic datasets with explicit 3D data (with simulated sensors) for outdoor environments are less common, although such sensors seem to be straightforward to include into self-driving car hardware. In their development of the \emph{SqueezeSeg} architecture, Wu et al.~\cite{DBLP:journals/corr/abs-1710-07368,DBLP:journals/corr/abs-1809-08495} added a LiDAR simulator to \emph{Grand Theft Auto V} and collected a synthetic dataset from the game. \emph{SynthCity} by Griffiths and Boehm~\cite{2019arXiv190704758G} is a large-scale open synthetic dataset which is basically a huge point cloud of an urban/suburban environment. It simulates the Mobile Laser Scanner (MLS) results with a \emph{Blender} plugin~\cite{10.1007/978-3-642-24031-7_20} and is specifically intended for pretraining deep neural networks.

...

Simulated environments rather than datasets are, naturally, also an important part of the outdoor navigation scene.

TORCS~\footnote{\url{http://torcs.sourceforge.net/}} (The Open Racing Car Simulator)~\cite{TORCS} is an open source 3D car racing simulator that started as a game for Linux in the late 1990s but became increasingly popular as a virtual simulation platform for driving agents and intelligent control systems for various car components. TORCS provides a sufficiently involved simulation of racing physics, including accurate basic properties (mass, rotational inertia), mechanical details (suspension types etc.), friction profiles of tyres, and a realistic aerodynamic model, so it is widely accepted as useful as a source of synthetic data. TORCS has become the basis for the annual Simulated Car Racing Championship~\cite{DBLP:journals/corr/abs-1304-1672} and has been used in hundreds of works on autonomous driving and control systems (see Section~\ref{sec:rl}).

CARLA (CAR Learning to Act)~\cite{Dosovitskiy17} is an open simulator for urban driving, developed as an open-source layer over Unreal Engine 4~\cite{Karis:2013}. Technically, it operates similarly to~\cite{7989092}, as an open source layer over Unreal Engine 4 that provides sensors in the form of RGB cameras (with customizable positions), ground truth depth maps, ground truth semantic segmentation maps with 12 semantic classes designed for driving (road, lane marking, traffic sign, sidewalk and so on), bounding boxes for dynamic objects in the environment, and measurements of the agent itself (vehicle location and orientation).

DeepDrive \cite{craig_quiter_2018_1248998}

VIVID (VIrtual environment for VIsual Deep learning), developed by Lai et al.~\cite{Lai:2018:VVE:3240508.3243653} tackles a more ambitious problem: adding people interacting in various ways and a much wider variety of synthetic environments, they present a universal dataset and simulator of outdoor scenes such as outdoor shooting, forest fires, drones patrolling a warehouse, pedestrian detection on the roads, and many more. VIVID is also based on the Unreal engine and uses the wide variety of assets available for it; for example, NPCs acting in the scenes are programmed using Blueprint, an Unreal scripting engine, and the human models are animated by the Unreal animation editor. VIVID provides the ability to record video simulations and can communicate with deep learning libraries via the TCP/IP protocol, through the Microsoft Remote Procedure Call (RPC) library developed for AirSim.

AirSim~\cite{airsim2017fsr}

...

% https://www.cvedia.com/solution/syncity/

\subsection{Indoor scenes and navigation}\label{sec:dataindoor}

Although, as we have seen in the previous section, the main emphasis of many influential applications remains in the outdoors, \emph{indoor navigation} is also an important field where synthetic datasets are required. The main problems remain the same---SLAM and navigation---but the potential applications are now more in the field of home robotics, industrial robots, and embodied AI~\cite{Mautz11,zhou17}. There are large-scale efforts to create real annotated datasets of indoor scenes~\cite{dai2017scannet,7298655,10.1007/978-3-642-33715-4_54,6751312,DBLP:journals/corr/abs-1709-06158,DBLP:journals/corr/abs-1808-10654}, but synthetic data is increasingly being used in the field~\cite{Zhang2019ASO}. 

Currently, the main synthetic dataset for indoor navigation is SUNCG\footnote{\url{http://suncg.cs.princeton.edu/}} presented by Song et al.~\cite{song2016ssc}. It contains over 45{,}000 different scenes (floors of private houses) with manually created realistic room layouts, 3D models of the furniture, realistic textures, and so on. All of the scenes are semantically annotated at the object level, and the dataset provides synthetic depth maps and volumetric ground truth data for the scenes. The original paper~\cite{song2016ssc} presented state of the art results in semantic scene completion, but, naturally, SUNCG has been used for many different tasks related to depth estimation, indoor navigation, SLAM, and others~\cite{Han2019DeepRL,Qi20173DGN,Chen20193DSS,Abbasi2018Deep3S,Ma2018LanguagedrivenSO}, and it often serves as the basis for scene understanding competitions~\cite{sumo2019}.

SUNCG has given rise to a number of simulation environments. Before SUNCG, we note the \emph{Gazebo} platform mentioned above~\cite{1389727} and the V-REP robot simulation framework~\cite{6696520} that not only provided visual information but also simulated a number of actual robot types, further simplifying control deployment and development.

MINOS by Savva et al.~\cite{savva2017minos} is a multimodal simulator for indoor navigation (later superceded by Habitat, see below). Wu et al.~\cite{DBLP:journals/corr/abs-1801-02209} made SUNCG into a full-scale simulation environment named House3D\footnote{\url{http://github.com/facebookresearch/House3D}}, with high-speed rendering suitable for large-scale reinforcement learning. In House3D, a virtual agent can freely explore 3D environments taken from SUNCG while providing all the modalities of SUNCG. House3D has been used, e.g., for the embodied question answering model by Das et al.~\cite{8575449}, where a robot is supposed to answer natural language questions by navigating an indoor environment. The AI2-THOR (The House Of inteRactions) framework~\cite{DBLP:journals/corr/abs-1712-05474} provides near photorealistic interactive environments with actionable objects (doors that can be opened, furniture that can be moved etc.) based on the \emph{Unity3D} game engine.

At the time of writing, the last (and very recent) major advance in the field is \emph{Habitat}, a simulation platform for embodied AI developed by Facebook researchers Savva et al.~\cite{habitat19arxiv}. Its simulator, called \emph{Habitat-Sim}, presents a number of important improvements over previous work that we have surveyed in this section:
\begin{itemize}	
	\item dataset support: \emph{Habitat-Sim} supports both synthetic datasets such as SUNCG~\cite{song2016ssc} and real-world datasets such as Matterport3D~\cite{DBLP:journals/corr/abs-1709-06158} and Gibson~\cite{DBLP:journals/corr/abs-1808-10654};
	\item rendering performance: \emph{Habitat-Sim} can render thousands of frames per second, 10-100x faster than previous simulators; the authors claim that ``it is often faster to generate images using \emph{Habitat-Sim} than to load images from disk''; this is important because simulation stops being a bottleneck in large-scale model training;
	\item humans-as-agents: humans can function as agents in the simulated environment, which allows to use real human behaviour in agent training and evaluation;
	\item accompanying library: the \emph{Habitat-API} library defines embodied AI tasks and implements metrics for easy agent development.
\end{itemize}
Savva et al. also provide a large-scale experimental study of various state of the art agents, arriving at the conclusion (counter to previous research) that reinforcement learning-based agents outperform SLAM-based ones, and RL agents generalize best across datasets, including the synthetic-to-real generalization from SUNCG to Matterport3D and Gibson. This is an important finding for synthetic data in indoor navigation, and we expect it to be confirmed in later studies; moreover, we expect \emph{Habitat} and its successors to become the new standard for indoor navigation and embodied AI research.

\subsection{Visual reasoning}\label{sec:datareason}

\begin{figure}[t]\centering
\input{tikz_clevr}

\caption{Sample visual reasoning questions from CLEVR; examples taken from~\cite{Johnson2017CLEVRAD}.}\label{fig:clevr}
\end{figure}

\emph{Visual reasoning} is the field of artificial intelligence where models are trained to reason and answer questions about visual data. It is usually studied in the form of visual question answering (VQA), when models are trained to answer questions about a picture such as ``What is the color of the small metal sphere?'' or ``Is there an equal number of balls and boxes?''.

There exist datasets for visual question answering based on real photographs, collected and validated by human labelers; they include the first large dataset called VQA~\cite{Agrawal2017} and its recent extension, VQA v2.0~\cite{Goyal2019}. However, the problem yields itself naturally to automated generation, so it is no wonder that synthetic datasets are important in the field.

The most important synthetic VQA dataset is CLEVR (Compositional Language and Elementary Visual Reasoning), created by Johnson et al. in a collaboration between Stanford and Facebook Research~\cite{Johnson2017CLEVRAD}. It contains 100K rendered images with scenes composed of simple geometric shapes and about 1M (853K unique) automatically generated questions about these images. The intention behind this dataset was to enable detailed analysis of VQA models, simplifying visual recognition and concentrating on reasoning about the objects.

In CLEVR, scenes are represented as scene graphs~\cite{Krishna2017,Johnson2015ImageRU}, where the nodes are objects annotated with attributes (shape, size, material, and color) and edges correspond to spatial relations between objects (``left'', ``right'', ``behind'', and ``in front''). A scene can be rendered based on its scene graph with randomized positions of the objects. The questions are represented as functional programs that can be executed on scene graphs, e.g., ``What color is the cube to the right of the white sphere?''. Different question types include querying attributes (``what color''), comparing attributes (``are they the same size''), existence (``are there any''), counting (``how many''), and integer comparison (``are there fewer''). When generating questions, special care is taken to ensure that the answer exists and is unique, and then the natural language question is generated with a relatively simple grammar. Figure~\ref{fig:clevr} shows two sample questions and their functional programs: on Fig.~\ref{fig:clevr}a the program is a simple chain of filters, and Fig.~\ref{fig:clevr}b adds a logical connective, which makes the graph a tree.

We also note a recently published COG dataset produced by Google Brain researchers~\cite{Yang2018ADA} that extends CLEVR's ideas to video processing. It also contains synthetic visual inputs and questions generated from functional programs, but now questions can refer to time (e.g., ``what is the color of the latest triangle?''). The authors also released a generator that can produce synthetic video-question pairs that are progressively more challenging and that have minimal response bias, an important problem for synthetic datasets (in this case, the generator begins with a balanced set of target responses and then generates videos and questions for them rather than the other way around).


